How "Multi" is Multi-Document Summarization?

The task of multi-document summarization (MDS) aims at models that, given multiple documents as input, are able to generate a summary that combines disperse information, originally spread across these documents. Accordingly, it is expected that both reference summaries in MDS datasets, as well as system summaries, would indeed be based on such dispersed information. In this paper, we argue for quantifying and assessing this expectation. To that end, we propose an automated measure for evaluating the degree to which a summary is ``disperse'', in the sense of the number of source documents needed to cover its content. We apply our measure to empirically analyze several popular MDS datasets, with respect to their reference summaries, as well as the output of state-of-the-art systems. Our results show that certain MDS datasets barely require combining information from multiple documents, where a single document often covers the full summary content. Overall, we advocate using our metric for assessing and improving the degree to which summarization datasets require combining multi-document information, and similarly how summarization models actually meet this challenge. Our code is available in https://github.com/ariecattan/multi_mds.

==> tables/abreviation.tex <==
\begin{table}[]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{p{0.6\textwidth}}
    \toprule
    
    % \multicolumn{2}{}{}
    \textbf{Document proposition}: The use of a Quadriceps tendon graft in primary ACL reconstruction leads to equal or better functional outcomes.\\ 
    
    \midrule 
    % \midrule 
    
    \textbf{Summary 1}: \textcolor{red}{QT} autograft represent a feasible option for primary ACL reconstruction. \quad \textbf{\textcolor{red}{\xmark}}  \\
    
    \midrule
    
    \textbf{Summary 2}: \textcolor{greenrgb}{Quadriceps Tendon} autograft represent a feasible option for primary ACL reconstruction. \quad \textbf{\textcolor{greenrgb}{\cmark}} \\
    \midrule
         
    \end{tabular}}
    \caption{Result of SuperPAL with and without abbreviation. The Document proposition is not aligned with Summary 1 because of the abbreviation \emph{QT}. When replacing the abbreviation by the original expression \emph{Quadriceps Tendon}, SuperPAL doesn't fail and predict that the propositions are aligned.}
    \label{tab:abr}
\end{table}


